Do Datasets Have Politics? Disciplinary Values in Computer Vision Dataset Development

Data is a crucial component of machine learning. The field is reliant on data to train, validate, and test models. With increased technical capabilities, machine learning research has boomed in both academic and industry settings, and one major focus has been on computer vision. Computer vision is a popular domain of machine learning increasingly pertinent to real-world applications, from facial recognition in policing to object detection for autonomous vehicles. Given computer vision's propensity to shape machine learning research and impact human life, we seek to understand disciplinary practices around dataset documentation - how data is collected, curated, annotated, and packaged into datasets for computer vision researchers and practitioners to use for model tuning and development. Specifically, we examine what dataset documentation communicates about the underlying values of vision data and the larger practices and goals of computer vision as a field. To conduct this study, we collected a corpus of about 500 computer vision datasets, from which we sampled 114 dataset publications across different vision tasks. Through both a structured and thematic content analysis, we document a number of values around accepted data practices, what makes desirable data, and the treatment of humans in the dataset construction process. We discuss how computer vision datasets authors value efficiency at the expense of care; universality at the expense of contextuality; impartiality at the expense of positionality; and model work at the expense of data work. Many of the silenced values we identify sit in opposition with social computing practices. We conclude with suggestions on how to better incorporate silenced values into the dataset creation and curation process.

==> archival-fig.tex <==
\begin{figure*}[htb!] 
    \centering
    \textbf{Number of Papers in Archival Venues}\par\medskip
    \includegraphics[width=\textwidth]{archival.png}
    \caption[A bar chart showing how many papers were published in archival venues (conferences, journals, etc.) versus non-archival venues (white papers, arxiv, personal websites, etc.).]{\small \new{A bar chart showing how many papers were published in archival venues (conferences, journals, etc.) versus non-archival venues (white papers, arxiv, personal websites, etc.). 105 papers were published in archival venues; 9 papers were not published in archival venues.}}
    \label{archival}
    \Description[A gray-scale bar chart showing how many dataset papers were published in archival venues (conferences, journals, etc.) versus non-archival venues (white papers, arxiv, personal websites, etc.).]{A gray-scale bar chart showing how many dataset papers were published in archival venues (conferences, journals, etc.) versus non-archival venues (white papers, arxiv, personal websites, etc.).}
\end{figure*}
\FloatBarrier
